Slow Roll Inflation: A Somehow Different Perspective

In this note we point out that, contrary to the standard point of view, slow roll inflation is due to high gravitational friction. We show that the requirement of slow roll coincides with the requirement of a flat scalar field potential in the case of minimally coupled scalar field. In this sense, the search for a successful inflationary theory may be more fruitful by shifting the focus on models with high gravitational friction. We review then a gravitational mechanism, the so called "Gravitationally Enhanced Friction" mechanism, such that high gravitational friction is dynamically generated during inflation allowing even steep (i.e. non-flat) scalar potential to inflate.

==> rjp_mathdefs.tex <==
%This file contains a hopefully ever growing collection of command shortcuts and even new LaTeX commands (especially for math mode),
% that are currently in use and accepted by Romanian Journal of Physics.

%Environment and general command shortcuts
\providecommand{\beq}[1][\@empty]{\def\@ttoken{#1}\begin{equation}\dbg@ut{\@ttoken}\ifx\@empty#1 \else\label{#1}\fi}
\newcommand{\eeq}{\end{equation}}
\newcommand{\beqn}{\begin{equation*}}
\newcommand{\eeqn}{\end{equation*}}

%elliptic Jacobi functions
\DeclareMathOperator{\sn}{sn}
\DeclareMathOperator{\cn}{cn}
\DeclareMathOperator{\dn}{dn}

%Mathematical operators and various symbols
\DeclareMathOperator{\ddiv}{div}
\DeclareMathOperator{\grad}{grad}
\DeclareMathOperator{\artanh}{artanh}
\DeclareMathOperator{\sech}{sech}
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\eps}{\ensuremath{\varepsilon}}
\newcommand{\cc}{\ifmmode\mathrm{cc.\;}\else\textrm{cc.~}\fi}
\newcommand{\ict}{\ifmmode\mathcal{C}\else\texttt{C}\fi}
\providecommand{\pd}{\ensuremath{\partial}}
\providecommand{\dd}{\ensuremath{\mathrm{d}}}
\providecommand{\id}{\ensuremath{\;\mathrm{d}}}

%bras and kets
\providecommand{\bra}[1]{\ensuremath{\left<#1\right|}}
\providecommand{\ket}[1]{\ensuremath{\left|#1\right>}}
%the \braket command is thought to be the matrix element of operator #1 for state #2 (left) and state #3 (right)
\providecommand{\braket}[3]{\ensuremath{\left<#2|#1|#3\right>}}

%Commands for multiple indexes around a central token #1
%The names derive from "front up-down, back up-down" of #1 (it better be read as "left up-down, right up-down") indicating 
%the order in which indexes are passed starting with #2 (left-up or front-up). The only cool stuff about these commands is 
%that it diminishes the space between up-down left indexes and the following token.
\newcommand{\fudbud}[5]{{\!\;}^{#2}_{#3}\!\!#1^{#4}_{#5}}
\newcommand{\fubu}[3]{{\!\;}^{#2}\!\!#1^{#3}}
\newcommand{\fdbd}[3]{{\!\;}_{#2}\!\!#1_{#3}}
\newcommand{\fdbu}[3]{{\!\;}_{#2}\!#1^{#3}}
\newcommand{\fubd}[3]{{\!\;}^{#2}\!#1_{#3}}

%put a small hat on operators!
\providecommand{\hatop}[1]{\ensuremath{\hat{\mathop{\operator@font #1}\nolimits}}}

%A small macro for generating uppercased letters of specific math font (mathfrak).
\let\op@format\mathfrak
%\let\op@format\mathcal
\def\op#1{%
 \ifnum`#1=\lccode`#1
  \expandafter\ensuremath\op@format{\uppercase{#1}}
 \else%
  \expandafter\ensuremath\op@format{#1}
 \fi%
}%

